Meson spectrum in the large $N$ limit

We present the result of our computation of the lowest lying meson masses for SU(N) gauge theory in the large $N$ limit (with $N_f/N\longrightarrow 0$). The final values are given in units of the square root of the string tension, and with errors which account for both statistical and systematic errors. By using 4 different values of the lattice spacing we have seen that our results scale properly. We have studied various values of $N$ (169, 289 and 361) to monitor the N-dependence of the most sensitive quantities. Our methodology is based upon a first principles approach (lattice gauge theory) combined with large $N$ volume independence. We employed both Wilson fermions and twisted mass fermions with maximal twist. In addition to masses in the pseudoscalar, vector, scalar and axial vector channels, we also give results on the pseudoscalar decay constant and various remormalization factors.

==> conclusion.tex <==
This paper summarizes the result of our analysis of meson masses in
pure SU(N) Yang-Mills theory in the limit of infinite number of colors
$N$. Quarks are not dynamical, but they produce 
nice observables of the Yang-Mills theory 

